XENON1T excess in local $Z_2$ DM models with light dark sector

Recently XENON1T Collaboration announced that they observed some excess in the electron recoil energy around a 2-3 keV. We show that this excess can be interpreted as exothermic scattering of excited dark matter (XDM), $XDM + e_{atomic} \rightarrow DM + e_{free}$ on atomic electron through dark photon exchange. We consider DM models with local dark $U(1)$ gauge symmetry that is spontaneously broken into its $Z_2$ subgroup by Krauss-Wilczek mechanism. In order to explain the XENON1T excess with the correct DM thermal relic density within freeze-out scenario, all the particles in the dark sector should be light enough, namely $\sim O(100)$ MeV for scalar DM and $\sim O(1-10)$ MeV for fermion DM cases. And even lighter dark Higgs $\phi$ plays an important role in the DM relic density calculation: $X X^\dagger \rightarrow Z' \phi$ for scalar DM ($X$) and $\chi \bar{\chi} \rightarrow \phi \phi$for fermion DM ($\chi$) assuming $m_{Z'} > m_\chi$. Both of them are in the $p$-wave annihilation, and one can easily evade stringent bounds from Planck data on CMB on the $s$-wave annihilations, assuming other dangerous $s$-wave annihilations are kinematically forbidden.

==> intro.tex <==
Recently XENON 1T Collaboration reported that they found electron recoil excess \cite{Aprile:2020tmw}.

After the accouncement of XENON1T Collaboration, there appeared a number of papers about this
excess \cite{Takahashi:2020bpq,OHare:2020wum,Kannike:2020agf,Alonso-Alvarez:2020cdv,Fornal:2020npv,Amaral:2020tga,Boehm:2020ltd,Harigaya:2020ckz,Bally:2020yid,Su:2020zny,Du:2020ybt,DiLuzio:2020jjp,Dey:2020sai,Chen:2020gcl,Bell:2020bes,AristizabalSierra:2020edu,Buch:2020mrg,Choi:2020udy,Paz:2020pbc,Lee:2020wmh,Cao:2020bwd,Robinson:2020gfu,Khan:2020vaf,Primulando:2020rdk,Nakayama:2020ikz,Gelmini:2020xir,Jho:2020sku,Bramante:2020zos,Baryakhtar:2020rwy,An:2020bxd,Zu:2020idx,Gao:2020wer,Budnik:2020nwz,Lindner:2020kko,Bloch:2020uzh,Chala:2020pbn,DeRocco:2020xdt,Dent:2020jhf,McKeen:2020vpf}.

In this paper, we interpret this electron recoil excess in terms of exothermic DM scattering on atomic 
electron bound to Xe. 

For the exothermic DM models, we consider both complex scalar and Dirac fermion DM models with
dark $U(1)$ gauge symmetry which is spontaneously broken into its $Z_2$ subgroup by 
Kraus-Wilczek mechanism \cite{}.  In this framework, the mass difference ($\Delta m$) between 
the DM and the. excited DM (XDM) is generated by dark Higgs mechanism, and there is no explicit 
violation of local gauge symmetry related with the presence of dark photon.  
On the other hand,  in a number of literature, $\Delta m$ is often introduced by hand in terms of 
dim-2 (3) operators for scalar (fermion) DM.  Then local gauge symmetry is broken explicitly but softly.  
Introducing dark gauge boson (or dark photon) in such a case would be theoretically inconsistent, 
since the current dark gauge fields couple is not a conserved current.  
There will appear some channels where high energy behavior of the scattering amplitudes violate
perturbative unitarity, in a similar way with the $W_L W_L \rightarrow W_L W_L$ scattering violates 
unitarity if $W$ boson mass is put in by hand.  One of the present authors  pointed out this issue 
in fermionic DM model (see Appendix A of Ref. \cite{}). 

Local $Z_2$ scalar and fermion DM models have been studied by authors for the $O(100)$ GeV 
-- O(1) TeV WIMP scenarios \cite{}.  In this paper we explore the same models for light DM mass 
$\lesssim O(1)$ GeV in order to evade the strong bounds from direct detections experiments searching 
for signals of DM scattering on various nuclei. In particular we will emphasize that the DM thermal 
relic density and the XENON1T  electron recoil excess with a few keV could be simultaneously 
accommodated if dark Higgs boson is light enough that 
${\rm DM} + {\rm XDM} \rightarrow Z^{' *} \rightarrow Z' \phi$ is kinematically open.  
This channel will play an important role when $m_{DM} < m_{Z'}$, as we  shall demonstrate 
in the following.  In order to explain the XENON1T excess in terms of 
${\rm XDM} e_{atomic} \rightarrow {\rm DM} e_{free}$ with a kinetic mixing, both dark photon and
(X)DM mass should be sub-GeV, more specifically $\sim O(100)$ MeV, in order to avoid the stringent 
bounds on the kinetic mixing parameter. For such a light DM, one has to consider the DM annihilation 
should be mainly in $p$-wave, and not in $s$-wave,  in order to avoid strong constraints from CMB 
\cite{}.  

For this purpose it is crucial to have dark Higgs $(\phi)$, since they can play a key roles in the $p$-wave 
annihilations of DM at freeze-out epoch:
\begin{eqnarray*}
X X^\dagger & \rightarrow & Z^{' *} \rightarrow Z^{'} \phi  , \\
\chi \overline{\chi} & \rightarrow & \phi \phi , 
\end{eqnarray*}
where $X$ and $\chi$ are complex scalar and Dirac fermion DM, respectively. 
At freeze-out epoch, the mass gap is too small ($\Delta m \ll T$) and we can consider DM as 
complex scalar or Dirac fermion.  In the present Universe,  we have $T \ll \Delta m$ and so we have 
to work in the two component DM picture.  It can not be emphasized enough that these channels 
would not be possible without dark Higgs $\phi$, and  it would be difficult to make the DM pair 
annihilation be dominated by the $p$-wave annihilation. 

